A Foundation for Spatio-Textual-Temporal Cube Analytics (Extended Version)

Large amounts of spatial, textual, and temporal data are being produced daily. This is data containing an unstructured component (text), a spatial component (geographic position), and a time component (timestamp). Therefore, there is a need for a powerful and general way of analyzing spatial, textual, and temporal data together. In this paper, we define and formalize the Spatio-Textual-Temporal Cube structure to enable combined effective and efficient analytical queries over spatial, textual, and temporal data. Our novel data model over spatio-textual-temporal objects enables novel joint and integrated spatial, textual, and temporal insights that are hard to obtain using existing methods. Moreover, we introduce the new concept of spatio-textual-temporal measures with associated novel spatio-textual-temporal-OLAP operators. To allow for efficient large-scale analytics, we present a pre-aggregation framework for the exact and approximate computation of spatio-textual-temporal measures. Our comprehensive experimental evaluation on a real-world Twitter dataset confirms that our proposed methods reduce query response time by 1-5 orders of magnitude compared to the No Materialization baseline and decrease storage cost between 97% and 99.9% compared to the Full Materialization baseline while adding only a negligible overhead in the Spatio-Textual-Temporal Cube construction time. Moreover, approximate computation achieves an accuracy between 90% and 100% while reducing query response time by 3-5 orders of magnitude compared to No Materialization.

==> figures/GammaDistribution.tex <==
%!TEX root = ../paper.tex

\begin{figure}[b]
	\centering
	\begin{tikzpicture}
		\begin{axis}[
			xlabel={K},
			ylabel={Values Count},
			xmode=log,
			log ticks with fixed point,
			xtick=data
		]
	
		\addplot[smooth, mark=*] coordinates {(10,26)	(20,21)	(50,33)	(100,15) (1000,5)};
		
		\end{axis}
	\end{tikzpicture}
	\caption{Top-K Vs Count}
	\label{fig:ValuesDistribution}
\end{figure}

==> figures/TopKAnalysis.tex <==
%!TEX root = ../paper.tex

\begin{figure}[b]
	\centering
	\scriptsize



\pgfplotsset{
	box plot width/.initial=1em,
	box plot/.style={
		/pgfplots/.cd,
		black,
		only marks,
		mark=-,
		mark size=\pgfkeysvalueof{/pgfplots/box plot width},
		/pgfplots/error bars/.cd,
		y dir=plus,
		y explicit,
	},
	box plot box/.style={
		/pgfplots/error bars/draw error bar/.code 2 args={%
			\draw  ##1 -- ++(\pgfkeysvalueof{/pgfplots/box plot width},0pt) |- ##2 -- ++(-\pgfkeysvalueof{/pgfplots/box plot width},0pt) |- ##1 -- cycle;
		},
		/pgfplots/table/.cd,
		y index=2,
		y error expr={\thisrowno{3}-\thisrowno{2}},
		/pgfplots/box plot
	},
	box plot top whisker/.style={
		/pgfplots/error bars/draw error bar/.code 2 args={%
			\pgfkeysgetvalue{/pgfplots/error bars/error mark}%
			{\pgfplotserrorbarsmark}%
			\pgfkeysgetvalue{/pgfplots/error bars/error mark options}%
			{\pgfplotserrorbarsmarkopts}%
			\path ##1 -- ##2;
		},
		/pgfplots/table/.cd,
		y index=4,
		y error expr={\thisrowno{2}-\thisrowno{4}},
		/pgfplots/box plot
	},
	box plot bottom whisker/.style={
		/pgfplots/error bars/draw error bar/.code 2 args={%
			\pgfkeysgetvalue{/pgfplots/error bars/error mark}%
			{\pgfplotserrorbarsmark}%
			\pgfkeysgetvalue{/pgfplots/error bars/error mark options}%
			{\pgfplotserrorbarsmarkopts}%
			\path ##1 -- ##2;
		},
		/pgfplots/table/.cd,
		y index=5,
		y error expr={\thisrowno{3}-\thisrowno{5}},
		/pgfplots/box plot
	},
	box plot median/.style={
		/pgfplots/box plot
	}
}

\begin{tikzpicture}
\begin{axis} 
[enlarge x limits=0.1,box plot width=0.5em, ymode=log, xtick=data, xticklabels = {10,20,50,100,200,500,1000}, xlabel={Materialized K}, ylabel={QRTs (msec)}, ymin=1,
height=3.5cm
]

\addplot [box plot median] table {testdata.dat};

\addplot [box plot box] table {testdata.dat};

\addplot [box plot top whisker] table {testdata.dat};

\addplot [box plot bottom whisker] table {testdata.dat};
\end{axis}
\end{tikzpicture}
	\caption{Materialized-K Vs QRT}
	\label{fig:TopKAnalysis}
\end{figure}

==> tables/accuracy_table.tex <==
%!TEX root = ../paper.tex

\begin{table}[t!]
	\footnotesize
	\begin{center}
		\caption{PAM\textquotesingle s Accuracy}
		\label{tab:accuracy}
		\begin{tabular}
			{||c||c|c|c|c|c||}
			\hline
			\multirow{2}{*}{\textbf{Query}} & \multicolumn{5}{c||}{Data Size in Millions} \\ \cline{2-6}
			 
			& 25 & 50 & 75 & 100 & 125 \\ \hline
		Q1 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 \\ \hline
		Q2 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 \\ \hline
		Q3 & 100.0 & 100.0 & 90.0 & 95.0 & 90.0\\ \hline
		Q4 & 92.3 & 100.0 & 100.0 & 100.0 & 100.0\\ \hline
		Q5 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 \\ \hline
		Q6 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0\\ \hline
		Q7 & 93.3 & 96.7 & 90.0 & 93.3 & 93.3\\ \hline
		Q8 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0\\ \hline
		\end{tabular}
	\end{center}
\end{table}

%\begin{table}[th!]
%	\begin{center}
%		\caption{Approximation Method\'s Accuracy Over Complete Dataset with varying Top-\text{k}}
%		\label{tab:accuracyNew}
%		\begin{tabular}
%			{||c||c|c|c|c||}
%			\hline
%			\multirow{2}{*}{\textbf{Query}} & \multicolumn{4}{c||}{Top-\textit{k}} \\ \cline{2-5}
%			
%			& \textbf{10} & \textbf{20} & \textbf{50} & \textbf{100} \\ \hline 
%			Q1 & 100 & 100 & 100 & 100 \\ \hline
%			Q2 & 100 & 100 & 100 & 100 \\ \hline
%			Q3 & 100 & 100 & 100 & 100 \\ \hline
%			Q4 & 100 & 100 & 100 & 100 \\ \hline
%			Q5 & 100 & 100 & 100 & 100 \\ \hline
%			Q6 & 100 & 100 & 100 & 100 \\ \hline
%			Q7 & 100 & 100 & 100 & 100 \\ \hline
%			Q8 & 100 & 100 & 100 & 100 \\ \hline
%		\end{tabular}
%	\end{center}
%\end{table}
